Performative Federated Learning: A Solution to Model-Dependent and Heterogeneous Distribution Shifts

We consider a federated learning (FL) system consisting of multiple clients and a server, where the clients aim to collaboratively learn a common decision model from their distributed data. Unlike the conventional FL framework that assumes the client's data is static, we consider scenarios where the clients' data distributions may be reshaped by the deployed decision model. In this work, we leverage the idea of distribution shift mappings in performative prediction to formalize this model-dependent data distribution shift and propose a performative federated learning framework. We first introduce necessary and sufficient conditions for the existence of a unique performative stable solution and characterize its distance to the performative optimal solution. Then we propose the performative FedAvg algorithm and show that it converges to the performative stable solution at a rate of O(1/T) under both full and partial participation schemes. In particular, we use novel proof techniques and show how the clients' heterogeneity influences the convergence. Numerical results validate our analysis and provide valuable insights into real-world applications.

==> Arxiv_ Performative FL (1)/convergence.tex <==
\section{Convergence Analysis} \label{sec:convergence}

In this section, we show that the \texttt{P-FedAvg} converges to the unique $\boldsymbol{\theta}^{PS}$ at a rate of $\mathcal{O}(1/T)$ under the assumptions made in Section \ref{sec:formulation}, which holds for all above-introduced schemes. The key observation is that for sufficiently small and decaying learning rates, the effect of $E$ steps is similar to a one-step update with a larger learning rate in the static case, as stated in \cite{li2020federated} without the performative setting. Therefore, given appropriate sampling and updating schemes that satisfy the above assumptions, the global update behaves similarly to the repeated performative SGD in \cite{ICML_2020_Perdomo_PP}. We also show that partial device participation makes the averaged parameter sequence $\{\overline{\boldsymbol{\theta}}^{t}\}$ have the same mean as but a larger variance than the full participation, where the variance can be controlled with carefully chosen learning rates. It's worth noting that the heterogeneity of clients plays a key role in the convergence analysis, which we elaborate on below.

{\bf Quantifying the heterogeneity.} The client heterogeneity can be quantified by the consensus error $\sum_{i=1}^N p_i \| \boldsymbol{\theta}_i^t - \overline{\boldsymbol{\theta}}^{t} \|_2^2$, which is dynamic due to the nature of performative prediction. It depends on both the shift mappings $\mathcal{D}_i$ and the decision parameters. After every broadcast, the heterogeneity leads to heterogeneous distribution shifts, causing heterogeneous local updates and eventually resulting in the consensus error. The $\varsigma$ value in Assumption \ref{asm:a5_bound_var_local_grad} is also a good indicator for heterogeneity.

Next, we will first present the convergence analysis of the full participation scheme and later extend the analysis to partial participation schemes. Due to the complexity of analysis in the performative setting, we define the following constants for ease of analysis and clarity of presentation.

{\bf Constants independent of system design.} \\
$ \overline{\epsilon} := \sum_{i=1}^N p_i \epsilon_i, ~~~~ \epsilon_{max} :=  \max_i \epsilon_i$,\\ 
$\Tilde{\mu} :=  \mu - (1+\delta) \overline{\epsilon} L$, ~~~ $\delta >0$, \\
    $c_1 :=  \big(L (1+\epsilon_{max})^2\big)/(2 \delta \overline{\epsilon})$,\\
    $c_2 := 4 \big[\sigma^2 + L^2(1+\epsilon_{max})^2\big]$, 
    \\
    $c_3:= 6\big[2\sigma^2+ 3 L^2(1+\epsilon_{\max})^2\big]$,
    \\
    $c_4:= 16\sigma^2+12\varsigma^2+ (8\sigma^2+12\varsigma^2)/\mathbb{E}\|\overline{\boldsymbol{\theta}}^0-\boldsymbol{\theta}^{PS}\|_2^2$,
    \\
    $c_5:=  (48\sigma^2+36\varsigma^2)\mathbb{E}\|\overline{\boldsymbol{\theta}}^0-\boldsymbol{\theta}^{PS}\|_2^2 +(24\sigma^2+36\varsigma^2)$.
    
{\bf Constants related to system design (e.g., $E, K$).} \\
    $c_6 := (2E^2+3E+1)\log (E+1)$,
    \\
    $\tilde{\eta}_0:=\Tilde{\mu} / \big(2\sigma^2+( c_1c_3  + c_2/6 ) c_4c_6\big)$,
   \\ 
    $\hat{\eta}_0 :=\Tilde{\mu}/ \big(2\sigma^2+( c_1c_3  + c_2/6 ) c_4(2E^2-E)\log E\big)$,
    \\
    $B :=2\sigma^2+ ( 4 c_1 \hat{\eta}_0 + 4 c_2 \hat{\eta}_0^2 )c_5(2E^2-E)\log E$ ,
\\
    $B_1 := 2 \sigma^2  + (4c_1 \tilde{\eta}_0 + 4c_2 \tilde{\eta}_0^2 +1/K) c_5 c_6 $,
    
    $B_2 := 2 \sigma^2 + \big(4c_1 \tilde{\eta}_0 + 4c_2 \tilde{\eta}_0^2 + \frac{N-K}{K(N-1)}\big )c_5c_6$.

\subsection{Convergence of Full Participation}

\begin{theorem}[Full Participation]\label{thm:full}Consider \texttt{P-FedAvg} with full participation and diminishing step size $\eta_t = \frac{2}{\Tilde{\mu}(t+\gamma)}$, where $\gamma = \max\left\{ \frac{2}{\Tilde{\mu} \hat{\eta}_0}, E,\frac{2}{\Tilde{\mu}} \sqrt{(4E^2+2E)c_3}\right\}$. 
   Under Assumption \ref{asm:a1_obj_str_conv}, \ref{asm:a2_obj_smooth}, 
\ref{asm:a3_map_sensitivity}, \ref{asm:a4_bound_var_sto_grad}, \ref{asm:a5_bound_var_local_grad}, the following holds %under a diminishing step size $\eta_t = \frac{2}{\Tilde{\mu}(t+\gamma)}$ where $\gamma = \max\{ \frac{2}{\Tilde{\mu} \hat{\eta}_0}, E,\frac{2}{\Tilde{\mu}} \sqrt{(4E^2+2E)c_3}\}$,
 %   then in full participation, we have for any $t$
    \begin{align*}
        \mathbb{E} [\| \overline{\boldsymbol{\theta}}^{t} - \boldsymbol{\theta}^{PS} \|^2_2]  
        \leq & \frac{\upsilon}{\gamma+t},~\forall t
    \end{align*}
    where $\upsilon=\max \left\{\frac{4 B}{ \Tilde{\mu}^2},\gamma \mathbb{E}\|\overline{\boldsymbol{\theta}}^0-\boldsymbol{\theta}^{PS}\|_2^2\right\}$.
    % and $\hat{\eta}_0, c_3, B$ are defined in Table \ref{table:constants}.
\end{theorem}

The proof of Theorem \ref{thm:full} can be found in Appendix \ref{appensec:full}. The key to the proof is that expected distance $\mathbb{E}\| \overline{\boldsymbol{\theta}}^t - \boldsymbol{\theta}^{PS} \|_2^2$ and expected consensus error $\sum_{i=1}^N p_i \mathbb{E}\| \boldsymbol{\theta}_i^{t-1} - \overline{\boldsymbol{\theta}}^{t} \|_2^2$ all depend on expected distance $\mathbb{E}\| \overline{\boldsymbol{\theta}}^{t-1} - \boldsymbol{\theta}^{PS} \|_2^2$ and expected consensus error $\sum_{i=1}^N p_i \mathbb{E}\| \boldsymbol{\theta}_i^{t-1} - \overline{\boldsymbol{\theta}}^{t-1} \|_2^2$ in the previous step. While we can establish a descent lemma for expected distance including the expected consensus error, it is impossible to establish one for expected consensus error, which makes it impossible to establish a joint descent lemma for expected distance and expected consensus error as in \cite{ArXiv_2022_Li_MPP}. Fortunately, consensus error will become zero at every aggregation step, which enables us to control expected consensus error at every step within a constant with a novel double-iteration technique under small enough step sizes. Then by relaxing the expected consensus error to the constant, we can establish a standard descent lemma in SGD analysis for expected distance. 

\subsection{Convergence of Partial Participation}

As mentioned in Section \ref{sec:formulation}, the partial participation scheme is more realistic  in federated learning \cite{ICLR_2020_Li_Convergence} and is of more interest since it reduces the stragglers' effect. 

We first present the convergence result of Scheme I.

\begin{theorem}[Partial Participation, Scheme I] \label{thm:partial_w_rep_convergence}Consider \texttt{P-FedAvg} with partial participation (scheme I) and a diminishing step size $\eta_t = \frac{2}{\Tilde{\mu}(t+\gamma)}$, where $\gamma = \max\left\{ \frac{2}{\Tilde{\mu} \tilde{\eta}_0}, E,\frac{2}{\Tilde{\mu}} \sqrt{(4E^2+10E+6)c_3}\right\}$.
   Under Assumption \ref{asm:a1_obj_str_conv}, \ref{asm:a2_obj_smooth}, \ref{asm:a3_map_sensitivity}, \ref{asm:a4_bound_var_sto_grad}, \ref{asm:a5_bound_var_local_grad}, the following holds %for a diminishing step size $\eta_t = \frac{2}{\Tilde{\mu}(t+\gamma)}$ where $\gamma = \max\{ \frac{2}{\Tilde{\mu} \tilde{\eta}_0}, E,\frac{2}{\Tilde{\mu}} \sqrt{(4E^2+10E+6)c_3}\}$, then for scheme I, we have for any $t$
    \begin{align*}
        \mathbb{E} [\| \overline{\boldsymbol{\theta}}^{t} - \boldsymbol{\theta}^{PS} \|^2_2]  
        \leq & \frac{\upsilon}{\gamma+t},~\forall t
    \end{align*}
    where $\upsilon=\max \left\{\frac{4 B_1}{ \Tilde{\mu}^2},\gamma \mathbb{E}\|\overline{\boldsymbol{\theta}}^0-\boldsymbol{\theta}^{PS}\|_2^2\right\}$.
    % and $\tilde{\eta}_0, c_3, B_1$ are defined in Table \ref{table:constants}.
\end{theorem}

Then we present the convergence result of Scheme II.
% the \emph{without replacement sub-scheme}. 
As discussed in Section \ref{sec:formulation}, we need probabilities $p_i = \frac{1}{N}, \forall i$ to ensure $\sum_{i \in \mathcal{S}_t} p_k \frac{N}{K}=1$.

\begin{theorem}[Partial Participation, Scheme II] \label{thm:partial_wo_rep_convergence}Consider \texttt{P-FedAvg} with partial participation (scheme II) and a diminishing step size $\frac{2}{\Tilde{\mu}(t+\gamma)}$, where $\gamma = \max\left\{ \frac{2}{\Tilde{\mu} \tilde{\eta}_0}, E,\frac{2}{\Tilde{\mu}} \sqrt{(4E^2+10E+6)c_5}\right\}$.
      Under Assumption \ref{asm:a1_obj_str_conv}, \ref{asm:a2_obj_smooth}, \ref{asm:a3_map_sensitivity}, \ref{asm:a4_bound_var_sto_grad}, \ref{asm:a5_bound_var_local_grad}, the following holds %for a diminishing step size $\frac{2}{\Tilde{\mu}(t+\gamma)}$ where $\gamma = \max\{ \frac{2}{\Tilde{\mu} \tilde{\eta}_0}, E,\frac{2}{\Tilde{\mu}} \sqrt{(4E^2+10E+6)c_5}\}$, then for scheme II, we have for any $t$
    \begin{align*}
        \mathbb{E} [\| \overline{\boldsymbol{\theta}}^{t} - \boldsymbol{\theta}^{PS} \|^2_2]  
        \leq & \frac{\upsilon}{\gamma+t},~\forall t
    \end{align*}
    where $\upsilon=\max \left\{\frac{4 B_2}{ \Tilde{\mu}^2},\gamma \mathbb{E}\|\overline{\boldsymbol{\theta}}^0-\boldsymbol{\theta}^{PS}\|_2^2\right\}$.
    % and $\tilde{\eta}_0, c_3, B_2$ are defined in Table \ref{table:constants}.
\end{theorem}

The proofs of Theorem \ref{thm:partial_w_rep_convergence} and \ref{thm:partial_wo_rep_convergence} can be found in Appendix \ref{appensec:partial}. Besides the technical difficulty as that of Theorem \ref{thm:full}, we also need to bound the variance of $\overline{\boldsymbol{\theta}}^t$ at the aggregation step. Fortunately, it can be bounded by the consensus error. Then by similar techniques as in the proof of Theorem \ref{thm:full}, we can establish a standard descent lemma in SGD analysis for the expected distance.

Scheme II requires $p_i = \frac{1}{N}, \forall i$, which violates the unbalanced nature of FL. One solution in \cite{ICLR_2020_Li_Convergence} is scaling the local objectives to $g_i(\boldsymbol{\theta}; \tilde{\boldsymbol{\theta}}) = p_i N f_i(\boldsymbol{\theta}; \tilde{\boldsymbol{\theta}})$, and then the global objective is a simple average of the scaled local objectives 
\begin{equation*}
    f(\boldsymbol{\theta}; \tilde{\boldsymbol{\theta}}) := \sum_{i=1}^N p_i f_{i}(\boldsymbol{\theta}; \tilde{\boldsymbol{\theta}}) = \frac{1}{N} \sum_{i=1}^N g_{i}(\boldsymbol{\theta}; \tilde{\boldsymbol{\theta}}).
\end{equation*}
We need to be careful with the Assumptions in Section \ref{sec:formulation} since scaling the objective will change those properties. The convergence theorems still hold if we replace $L, \mu, \sigma, \varsigma$ with $L' := q_{max} L, \mu' := q_{min} \mu, \sigma' := \sqrt{q_{max}} \sigma, \varsigma' := \sqrt{q_{max}} \varsigma$, where $q_{max} := N \cdot \max_i p_i, q_{min} := N \cdot \min_i p_i$.

\subsection{Discussions on the Algorithm and Solution} \label{subsec:discussion_alg_sol}
We will only discuss with respect to the aggregation step in this sub-section for convenience, denoted as $T \in \mathcal{I}_E$, then we can simply use $\frac{T}{E}$ when dividing $E$. Note for a general step $t$, we only need to use $\lfloor \frac{t}{E}\rfloor$ to obtain an integer.

\textbf{Choice of $E$.} We are interested in the total time we need to achieve an $\epsilon$ accuracy, and how this total time changes with $E$. We use our results in Theorem \ref{thm:full}, \ref{thm:partial_w_rep_convergence}, and \ref{thm:partial_wo_rep_convergence}, and denote $T_{\epsilon} := \frac{\upsilon}{\epsilon} - \gamma$ as the number of computation steps that is sufficient to guarantee an $\epsilon$-accuracy. To connect $T_{\epsilon}$ to the total time needed, suppose the expected time for each communication step is $C$ times the expected time of each computation step, then the total time required for $\epsilon$-accuracy is linear in $T_{\epsilon} + C \cdot \frac{T_{\epsilon}}{E}$. Below we separately analyze the influence of $E$ on $\frac{T_{\epsilon}}{E}$ and $T_{\epsilon}$, and then discuss how to choose the optimal $E$ for different $C$ values. 

Let $B_0:=B$ in Theorem \ref{thm:full} for full participation and $\gamma_i$ ($i=0,1,2$) denotes the $\gamma$ in Theorem \ref{thm:full}, \ref{thm:partial_w_rep_convergence}, and \ref{thm:partial_wo_rep_convergence} respectively. Then in Theorem \ref{thm:full}, \ref{thm:partial_w_rep_convergence}, and \ref{thm:partial_wo_rep_convergence}, $T_\epsilon$ is dominated by $\mathcal{O}\big(4 B_i/\Tilde{\mu}^2 +\gamma_i \mathbb{E} [\| \overline{\boldsymbol{\theta}}^{0} - \boldsymbol{\theta}^{PS} \|^2_2]\big)$ where $i=0,1,2$. From the definition, we know that $B_i$ ($i=0,1,2$) is almost a constant w.r.t. $E$ and $\gamma_i$ is of $\mathcal{O}(E^2\log E)$. This means that when $E$ grows, the total update steps to reach $\epsilon$-accuracy, $T_\epsilon$ will grow, while the number of aggregation steps needed, $\frac{T_\epsilon}{E}$ will first grow and then decrease. 

Now we consider $T_{\epsilon} + C \cdot \frac{T_{\epsilon}}{E}$, the total time needed to reach $\epsilon$-accuracy. From the above analysis, we know it is of order $\mathcal{O}(E^2\log E)+ C\cdot \mathcal{O}(E\log E)+C\cdot \mathcal{O}(\log E/E)$.
When communication is fast, i.e., $C$ is small, $\mathcal{O}(E^2\log E)$ is the dominating term, and we can focus more on the number of computation iterations $T_\epsilon$, and smaller $E$ values are preferable. However, when $C$ is large, $C\cdot \mathcal{O}(E\log E)+C\cdot \mathcal{O}(\log E/E)$ becomes the dominating term, and we should focus more on the number of communication rounds $\frac{T_\epsilon}{E}$ and some middle $E$ values are preferable.

\textbf{Choice of $K$.} Again $T_{\epsilon}$ is dominated by $\mathcal{O}\big(4 B_i/\Tilde{\mu}^2 +\gamma_i \mathbb{E} [\| \overline{\boldsymbol{\theta}}^{0} - \boldsymbol{\theta}^{PS} \|^2_2]\big)$ where $i=1,2$. Then by the formulae of $B_i$ ($i=1,2$), we know $T_\epsilon$ monotonically decreases with $K$, but the total communication time increases with $K$ due to more severe stragglers' effect. Generally, as we show in Theorem \ref{thm:partial_w_rep_convergence} and \ref{thm:partial_wo_rep_convergence}, the convergence rate has a weak dependence on $K$. We have empirically observed this phenomenon in Figure \ref{fig:impactofk:a}. Therefore, we can set $\frac{K}{N}$ to an appropriate small value to reduce the straggler's effect while keeping the convergence rate.

\textbf{Choice of sampling schemes.} We formalize the two sampling schemes in Section \ref{sec:formulation} and show their convergence properties in Theorem \ref{thm:partial_w_rep_convergence} and \ref{thm:partial_wo_rep_convergence}. We note that Scheme I has a desirable property that it naturally supports unbalanced clients, so if the server has control over the sampling, Scheme I should be chosen. 

But as discussed in \cite{ICLR_2020_Li_Convergence}, sometimes the server may have no control over the sampling and simply use the first $K$ received results for update. In this case, if the reception times from each client are IID random variables, we can treat this process as uniformly sampling $K$ out of $N$ at random without replacement. Theorem \ref{thm:partial_wo_rep_convergence} showed the convergence, and the discussion on scaling the objectives provides instructions on how to make the system work with arbitrary initial $p_1, \dots, p_N$ values. However, it's worth noting that when $p_1, \dots, p_N$ are highly non-uniform, the corresponding  $L', \sigma', \varsigma'$ values will be much larger than from $L, \sigma, \varsigma$, and $\mu'$ will be much smaller than $\mu$. Then by the formula of $\hat{\eta}_0$ and $\Tilde{\eta}_0$, we have to use much smaller starting learning rates and thus slower convergence. However, such a small learning rate may cause the model to fail to train at all. We also empirically show this in \cref{fig:highvarp}. 

However, an interesting observation is that when $p_i = \frac{1}{N}$, we empirically show in Figure \ref{fig:impactofh} and \ref{fig:credit}, Scheme II slightly outperforms Scheme I.

\textbf{Learning rate decay.} The learning rate decay is a necessity for stochastic gradient descent (SGD) to converge, even when clients have static, independent and individually distributed (IID) data. The decay is used in \cite{ArXiv_2022_Li_MPP} in decentralized performative prediction and the necessity for such decay is proved in \texttt{FedAvg} with static, non-IID clients. We also empirically show that constant learning rates fail to converge in \cref{fig:learningrate}.

\textbf{$\boldsymbol{\theta}^{PS}$ and $\boldsymbol{\theta}^{PO}$.} Here we discuss the relationship between the $\boldsymbol{\theta}^{PS}$ and $\boldsymbol{\theta}^{PO}$ solutions more in depth. In the strategic learning setting, \cite{ICML_2020_Perdomo_PP} showed that  $\boldsymbol{\theta}^{PO}$ is the Stackelberg equilibrium. It's worth noting that  $\boldsymbol{\theta}^{PS}$ is not merely an approximation to $\boldsymbol{\theta}^{PO}$, but a natural convergence point of the best response dynamics (BRD). More specifically, when the clients and the decision maker have no information about others' utilities, backward induction is unavailable, and playing the Stackelberg equilibrium is unrealistic. In this case, treating others' strategies in the previous time step as constants, and optimizing one's own strategy accordingly is a rational strategy. Such an optimization step is a best response, and in multi-round sequential strategic learning problems \cite{NEURIPS_2021_Zrnic}, the best responses can form the BRD, and $\boldsymbol{\theta}^{PS}$ is {\bf the convergence point of the BRD}. Although the decision maker's natural best response step is a risk minimization step, the gradient-based \texttt{P-FedAvg} can find the same $\boldsymbol{\theta}^{PS}$. Another interesting observation of $\boldsymbol{\theta}^{PS}$ is that if we remove the sequential decision nature, then $\{ \boldsymbol{\theta}^{PS}, \mathcal{D}_1(\boldsymbol{\theta}^{PS}), \dots, \mathcal{D}_N(\boldsymbol{\theta}^{PS}) \}$ is a {\bf Nash equilibrium} since no participant has an incentive to unilaterally deviate. 

==> Arxiv_ Performative FL (1)/formulation.tex <==
\section{Problem Formulation} \label{sec:formulation}

In this section, we formulate the performative federated learning problem, define the learning objective, and introduce our performative federated learning algorithm to optimize the objective function. 

To help with the understanding of performative federated learning, we first recall the performative prediction problem \cite{ICML_2020_Perdomo_PP}. Consider a typical loss minimization problem where the data distribution experiences a shift induced by the model parameter, expressed as a mapping $\mathcal{D}(\boldsymbol{\theta})$. The objective function is thus given by
\begin{equation*}
    f(\boldsymbol{\theta}) := \mathbb{E}_{Z \sim \mathcal{D}(\boldsymbol{\theta})}[\ell(\boldsymbol{\theta};Z)],
\end{equation*}
where $\ell$ denotes the loss function. Then the performative optimal (PO) solution is
%\begin{equation*}
 $  \boldsymbol{\theta}^{PO} := \arg \min_{\boldsymbol{\theta}} f(\boldsymbol{\theta})$.
%\end{equation*}
\cite{ICML_2020_Perdomo_PP} also introduces a second,  decoupled objective function, also called the performatively stable (PS) model, which separates decision parameters ($\boldsymbol{\theta}$) from deployed parameters ($\Tilde{\boldsymbol{\theta}}$): 
\begin{equation*}    f(\boldsymbol{\theta};\Tilde{\boldsymbol{\theta}}) := \mathbb{E}_{Z \sim \mathcal{D}(\Tilde{\boldsymbol{\theta}})}[\ell(\boldsymbol{\theta};Z)]. 
\end{equation*}
Minimizing this objective 
 achieves minimal risk for the distribution  induced by the deployed parameters, eliminating  the need for
retraining, which makes it more practical. 
The PS solution is defined as
%\begin{equation*}
$    \boldsymbol{\theta}^{PS} := \arg \min_{\boldsymbol{\theta}} f(\boldsymbol{\theta};\boldsymbol{\theta}^{PS})$. 
%\end{equation*}
\cite{ICML_2020_Perdomo_PP} showed that $\boldsymbol{\theta}^{PS} \neq \boldsymbol{\theta}^{PO}$ in general. We next consider a distributed setting and introduce performative federated learning. 

\subsection{System Settings and Objectives} \label{subsec:system_settings_objectives}
Consider a system with $N$ clients and a server, where the clients have feature distributions as $\mathcal{D}_i(\boldsymbol{\theta})$, supported on $\mathcal{Z} \subseteq \mathbb{R}^M$, and $\boldsymbol{\theta} \in \mathbb{R}^m$ denotes the decision (model) parameters deployed on the $i$-th client. We consider the general case where clients can have heterogeneous distributions $\mathcal{D}_i(\boldsymbol{\theta}) \neq \mathcal{D}_j(\boldsymbol{\theta})$, and each client represents a $p_i > 0$ fraction of the total data population, $\sum_{i=1}^N p_i = 1$. 

The system aims to minimize the weighted average loss across all agents, which is given by the performative optimal objective as follows 
\begin{equation} \label{eq:theta_PO}
    \boldsymbol{\theta}^{PO} := \arg \min_{\boldsymbol{\theta} \in \mathbb{R}^m} \sum_{i=1}^N p_i \mathbb{E}_{Z_i \sim \mathcal{D}_i(\boldsymbol{\theta})}[\ell(\boldsymbol{\theta};Z_i)].
\end{equation}

We note that our objective reduces to that in \cite{ArXiv_2022_Li_MPP} when $p_i = \frac{1}{N}$ for all $i$. This objective can typically model the strategic learning problem with different sub-populations in the system, where each client corresponds to a sub-population. Each sub-population may differ in some attributes so that they respond to the decision parameters differently, e.g., due to different action costs \cite{Milli2019, Hu2019, braverman2020role, Zhang_2022_ICML, EC_22_Jin}. The decision maker uses a common decision rule for the entire population and aims to minimize the expected loss, and $p_i$ represents the population fraction of each sub-population.
Correspondingly, the decoupled/performative stable objective is
\begin{equation*}
    f_{i}(\boldsymbol{\theta} ; \tilde{\boldsymbol{\theta}}) := \mathbb{E}_{Z_i \sim \mathcal{D}_i(\tilde{\boldsymbol{\theta}})}[\ell(\boldsymbol{\theta}; Z_i)], f(\boldsymbol{\theta};\tilde{\boldsymbol{\theta}}) := \sum_{i=1}^N p_i f_{i}(\boldsymbol{\theta}; \tilde{\boldsymbol{\theta}}),     
\end{equation*}
where the first argument denotes the client's decision parameter,
and the second argument the deployed parameters, which determine the distribution of the samples together with 
$\mathcal{D}_i(\cdot)$. The PS solution is 
\begin{equation}
    \begin{aligned}
        \boldsymbol{\theta}^{PS} := &~ \arg \min_{\boldsymbol{\theta}} \sum_{i=1}^N p_i \mathbb{E}_{Z_i \sim \mathcal{D}_i(\boldsymbol{\theta}^{PS})}[\ell(\boldsymbol{\theta};Z_i)]\\
        = &~ \arg \min_{\boldsymbol{\theta}} f(\boldsymbol{\theta};\boldsymbol{\theta}^{PS}).
    \end{aligned}
\end{equation}
Note that this is a fixed point equation with $\boldsymbol{\theta}^{PS}$ as a fixed point.

\subsection{Key Assumptions}

We make the following assumptions similar to \cite{ArXiv_2022_Li_MPP,ICML_2020_Perdomo_PP}:
\begin{assumption}[Strong Convexity] \label{asm:a1_obj_str_conv}
  \label{asm:convex} Given any $\tilde{\boldsymbol{\theta}} \in \mathbb{R}^m$, $f(\cdot, \tilde{\boldsymbol{\theta}})$ is $\mu$-strongly convex in $\boldsymbol{\theta}$, i.e., $
        f(\boldsymbol{\theta}';\tilde{\boldsymbol{\theta}}) \geq f(\boldsymbol{\theta};\tilde{\boldsymbol{\theta}}) + \langle \nabla f(\boldsymbol{\theta};\tilde{\boldsymbol{\theta}}) , \boldsymbol{\theta}' - \boldsymbol{\theta} \rangle + \frac{\mu}{2} \| \boldsymbol{\theta}' - \boldsymbol{\theta} \|_2^2, \forall \boldsymbol{\theta}', \boldsymbol{\theta} \in \mathbb{R}^K$.
\end{assumption}

In Assumption \ref{asm:a1_obj_str_conv}, we do not require strong convexity for every single $f_i$ but only the weighted average $f$.

\begin{assumption}[Smoothness] \label{asm:a2_obj_smooth}
     The loss function $\ell(\boldsymbol{\theta}; z)$ is $L$-smooth, i.e., 
    \begin{equation*}
        \|\nabla \ell(\boldsymbol{\theta}; \boldsymbol{z}) - \nabla \ell(\boldsymbol{\theta}'; \boldsymbol{z}')\|_2 \leq L (\| \boldsymbol{\theta}- \boldsymbol{\theta}'\|_2 + \|\boldsymbol{z}-\boldsymbol{z}'\|_2).
    \end{equation*}
\end{assumption}

\begin{assumption}[Distribution Mapping Sensitivity] \label{asm:a3_map_sensitivity} \label{asm:sensitive} For any $i = 1,\dots, n$ there exists $\epsilon_i > 0$ such that
    \begin{equation*}
    \mathcal{W}_1(\mathcal{D}_i(\boldsymbol{\theta}), \mathcal{D}_i(\boldsymbol{\theta}')) \leq \epsilon_i \|\boldsymbol{\theta} - \boldsymbol{\theta}'\|_2, ~~ \forall \boldsymbol{\theta}', \boldsymbol{\theta} \in \mathbb{R}^m,
    \end{equation*}
    where $\mathcal{W}_1(\mathcal{D}, \mathcal{D}'))$ is the 1-Wasserstein distance under $L_2$ norm between the distributions $\mathcal{D}, \mathcal{D}'$.
\end{assumption}

Assumption \ref{asm:a2_obj_smooth} and \ref{asm:a3_map_sensitivity} together induce the smoothness of $f_i(\cdot, \cdot)$, which is a result of Lemma 2.1 in \cite{drusvyatskiy2022stochastic} and will be used in the later proofs. 
\begin{lemma}[Continuity of $\triangledown f_i$] \label{lemma:fi_grad_continuity}
    Under Assumption \ref{asm:a2_obj_smooth} and \ref{asm:a3_map_sensitivity}, for any $\boldsymbol{\theta}_0, \boldsymbol{\theta}_1, \boldsymbol{\theta}, \hat{\boldsymbol{\theta}} \in \mathbb{R}^m$,
    \begin{equation*}
        \|\nabla f_i(\boldsymbol{\theta}_0; \boldsymbol{\theta}) 
        - \nabla f_i(\boldsymbol{\theta}_1; \hat{\boldsymbol{\theta}})\|_2 \leq
        L \|\boldsymbol{\theta}_0 - \boldsymbol{\theta}_1 \|_2 + L \epsilon_i \|\boldsymbol{\theta} - \hat{\boldsymbol{\theta}} \|_2.
    \end{equation*}
\end{lemma}

We introduce the following assumptions specifically made in decentralized performative predictions \cite{ArXiv_2022_Li_MPP}.

\begin{assumption}[Stochastic Gradient Variance Bound] \label{asm:a4_bound_var_sto_grad}
    For any $i=1, \dots, N$ and $\boldsymbol{\theta} \in \mathbb{R}^m$, there exists $\sigma \geq 0$ such that 
    \begin{equation*}
        \mathbb{E}_{Z_i \sim \mathcal{D}_i(\boldsymbol{\theta})}\| \nabla \ell (\boldsymbol{\theta}; Z_i) - \nabla f_i(\boldsymbol{\theta}; \boldsymbol{\theta}) \|_2^2 \leq \sigma^2 (1 + \|\boldsymbol{\theta} - \boldsymbol{\theta}^{PS}\|_2^2).
    \end{equation*}
\end{assumption}

\begin{assumption}[Local Gradient Bound] \label{asm:a5_bound_var_local_grad}
For any $i=1, \dots, N$ and $\boldsymbol{\theta} \in \mathbb{R}^m$, there exists $\varsigma \geq 0$ such that 
    \begin{equation*}
        \left\|\nabla f(\boldsymbol{\theta} ; \boldsymbol{\theta})-\nabla f_i(\boldsymbol{\theta} ; \boldsymbol{\theta})\right\|_2^2 \leq \varsigma^2(1+\|\boldsymbol{\theta}-\boldsymbol{\theta}^{PS}\|_2^2).
    \end{equation*}
\end{assumption}

Here we elaborate on Assumption \ref{asm:a5_bound_var_local_grad}, and explain reasons for using it over another commonly used assumption in federated learning \cite{ICLR_2020_Li_Convergence}, which is 
\begin{equation}\label{asm:uniform_gradnorm_bound}
    \mathbb{E}_{Z_i \sim \mathcal{D}_i(\boldsymbol{\theta})} [ \| \nabla \ell(\boldsymbol{\theta} ; Z_i) \|_2^2 ] \leq G^2.
\end{equation}
First, it can be shown that \eqref{asm:uniform_gradnorm_bound} implies Assumption \ref{asm:a5_bound_var_local_grad}, thus Assumption \ref{asm:a5_bound_var_local_grad} is weaker than \eqref{asm:uniform_gradnorm_bound}. To see this: when \eqref{asm:uniform_gradnorm_bound} holds, let $\varsigma^2 = 4G^2$, then $\left\|\nabla f(\boldsymbol{\theta} ; \boldsymbol{\theta})-\nabla f_i(\boldsymbol{\theta} ; \boldsymbol{\theta})\right\|_2^2 \leq 2 \left\|\nabla f(\boldsymbol{\theta} ; \boldsymbol{\theta})\|_2^2 + 2 \| \nabla f_i(\boldsymbol{\theta} ; \boldsymbol{\theta})\right\|_2^2 \leq 4 G^2 = \varsigma^2$.

We further give a concrete example where \eqref{asm:uniform_gradnorm_bound} does not hold but Assumption \ref{asm:a5_bound_var_local_grad} holds. 

%{\bf Example.} 
\begin{example}
Suppose we have a two-client Gaussian mean estimation problem $\ell(\theta, Z) = \frac{1}{2}(\theta-Z)^2$ where $\theta, Z\in \mathbb{R}$, $\mathcal{D}_1(\theta) = \mathcal{N}(\frac{1}{2}\theta, \sigma^2)$, $\mathcal{D}_2(\theta) = \mathcal{N}(-\frac{1}{2}\theta, \sigma^2)$, and $p_1 = p_2 = \frac{1}{2}$. Then $\mathbb{E}_{Z_1 \sim \mathcal{D}_1(\theta)} [ \| \nabla \ell(\theta ; Z_1) \|_2^2 ] = \mathbb{E}_{Z_1 \sim \mathcal{D}_1(\theta)}[(\theta-Z_1)^2] = \sigma^2 + (\mathbb{E}_{Z_1 \sim \mathcal{D}_1(\theta)}[\theta-Z_1])^2 = \frac{1}{4} \theta^2 + \sigma^2$ and $\mathbb{E}_{Z_2 \sim \mathcal{D}_2(\theta)} [ \| \nabla \ell(\theta ; Z_2) \|_2^2 ] = \frac{9}{4} \theta^2 + \sigma^2$ which all go to infinity when $\theta$ goes to infinity. Thus \eqref{asm:uniform_gradnorm_bound} does not hold. On the other hand, $\nabla f_1(\theta; \theta)=\frac{1}{8} \theta$, $\nabla f_2(\theta; \theta)=\frac{9}{8} \theta$, and $\nabla f(\theta;\theta)= \frac{5}{8} \theta$, $\theta^{PS} = 0$, then by taking $\varsigma=\frac{1}{2}$, we can verify Assumption \ref{asm:a5_bound_var_local_grad} holds.
\end{example}

Secondly, \eqref{asm:uniform_gradnorm_bound} also implies Assumption \ref{asm:a4_bound_var_sto_grad}: when \eqref{asm:uniform_gradnorm_bound} holds, letting $\sigma^2 = G^2$ leads to $\mathbb{E}[\| \nabla l (\boldsymbol{\theta}; Z_i) - \nabla f_i(\boldsymbol{\theta}, \boldsymbol{\theta}) \|_2^2] \le \mathbb{E}[\| \nabla l (\boldsymbol{\theta}; Z_i) \|_2^2] \le G^2 = \sigma^2$. On the other hand, Assumption \ref{asm:a5_bound_var_local_grad} does not imply Assumption \ref{asm:a4_bound_var_sto_grad}.

It turns out that Assumption \ref{asm:a5_bound_var_local_grad} better characterizes the system heterogeneity, as we show how the heterogeneity impacts  convergence (more details are in Theorem \ref{thm:full}, \ref{thm:partial_w_rep_convergence}, and \ref{thm:partial_wo_rep_convergence}). 


\subsection{Properties of the PS Solution}
Define the \textit{average sensitivity}  as $\overline{\epsilon} := \sum_{i=1}^N p_i \epsilon_i$, and the mapping $\Phi(\boldsymbol{\theta}) := \arg \min_{\boldsymbol{\theta}' \in \mathbb{R}^m} f(\boldsymbol{\theta}', \boldsymbol{\theta})$. Then we can establish the existence and uniqueness of the PS solution.
\begin{proposition}[Uniqueness of $\boldsymbol{\theta}^{PS}$]\label{prop:unique_PS}
     Under Assumptions \ref{asm:a1_obj_str_conv}, \ref{asm:a2_obj_smooth} and \ref{asm:a3_map_sensitivity}, 
    if $\overline{\epsilon} %:= \sum_{i=1}^N p_i \epsilon_i 
    < \mu/L$, then $\Phi(\cdot)$ is a contraction mapping with the unique fixed point $\boldsymbol{\theta}^{PS} = \Phi(\boldsymbol{\theta}^{PS})$; if $\overline{\epsilon} \ge \mu/L$, then there is an instance where any sequence generated by $\Phi(\cdot)$ will diverge.
\end{proposition}

Proposition \ref{prop:unique_PS} establishes a sufficient and necessary condition for the existence of $\boldsymbol{\theta}^{PS}$, similar to \cite{ArXiv_2022_Li_MPP}. This condition only depends on the average sensitivity $\overline{\epsilon}$, which implies that we may still have a unique performative stable solution $\boldsymbol{\theta}^{PS}$ for the whole system even if certain clients do not. The following proposition further validates the quality of $\boldsymbol{\theta}^{PS}$ in terms of its distance to $\boldsymbol{\theta}^{PO}$.

\begin{proposition}[Distance $\|\boldsymbol{\theta}^{PO}-\boldsymbol{\theta}^{PS} \|_2$ Bound]\label{prop:PS_PO_distance} %Let $\overline{\epsilon} := \sum_{i=1}^N p_i \epsilon_i$.
Under Assumption \ref{asm:a1_obj_str_conv} and \ref{asm:a3_map_sensitivity}, suppose that the loss $\ell(\boldsymbol{\theta}; Z)$ is $L_z$-Lipschitz in $Z$, then for every performative stable solution $\boldsymbol{\theta}^{PS}$ and every performative optimal solution $\boldsymbol{\theta}^{PO}$, we have
$
\|\boldsymbol{\theta}^{PS} -\boldsymbol{\theta}^{PO}\|_2 \le \big(2L_z  \overline{\epsilon}\big)/\mu.
$
\end{proposition}
 The proofs of Proposition \ref{prop:unique_PS} and \ref{prop:PS_PO_distance} are in Appendix \ref{appensec:prop}.

\subsection{The \texttt{P-FedAvg} Algorithm}

In \texttt{P-FedAvg}, the clients communicate with the server  every $E$ local updates. Denote $\mathcal{I}_{E} := \{nE | n = 1, 2 , \dots\}$ as the set of aggregation steps. Next, we formalize the full and partial participation schemes of the proposed {\bf \texttt{P-FedAvg}}.

\textbf{Full client participation.} All clients communicate with the server at every aggregation step and update the local models $\boldsymbol{\theta}_i^{t+1}$ based on the following: let $Z_i^{t+1} \sim \mathcal{D}_i(\boldsymbol{\theta}_i^{t})$, then
\begin{align*}
    & \boldsymbol{w}_i^{t+1} = \boldsymbol{\theta}_i^{t} 
    - \eta_{t} \nabla \ell(\boldsymbol{\theta}_i^t; Z_i^{t+1}); \\
    & \boldsymbol{\theta}_i^{t+1} = \begin{cases}
        & \sum_{j=1}^N p_j \boldsymbol{w}_j^{t+1} ~~~~\text{if}~ t+1 \in \mathcal{I}_{E} \\
        & \boldsymbol{w}_i^{t+1} ~~~~~~~~~~~~~~~~~~\text{o.w.}
    \end{cases}
\end{align*}
\textbf{Partial client participation.} A more realistic setting that does not require the response of all clients' output at every aggregation step. In this case, the central server only collects the outputs of the first $K<N$ responded clients  at the aggregation step. Denote  the first $K<N$ responded clients in $t$-th step as a size-$K$ set $\mathcal{S}_t:=\{i_1,\ldots, i_K\}\in [N]$. Let $Z_i^{t+1} \sim \mathcal{D}_i(\boldsymbol{\theta}_i^{t})$, then
\begin{align*}
    & \boldsymbol{w}_i^{t+1} = \boldsymbol{\theta}_i^{t} 
    - \eta_{t} \nabla \ell(\boldsymbol{\theta}_i^t; Z_i^{t+1}); \nonumber \\
    & \boldsymbol{\theta}_i^{t+1} = \begin{cases}
        & \left(\begin{array}{l}
             \text {samples } \mathcal{S}_{t+1}, \text {and}   \\
             \text{average}\left\{\boldsymbol{w}_{t+1}^k\right\}_{k \in \mathcal{S}_{t+1}}
        \end{array}\right) ~~\text{if}~ t+1 \in \mathcal{I}_{E} \\
        & ~~\boldsymbol{w}_i^{t+1} ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\text{o.w.}
    \end{cases}
\end{align*}
We further consider two schemes of partial participation:
\begin{enumerate}
    \item (\textbf{Scheme I}) The server establishes $\mathcal{S}_{t+1}$ by \textbf{\textit{i.i.d. with replacement}} sampling an index $k \in\{1, \cdots, N\}$ with probabilities $p_1, \cdots, p_N$ for $K$ times. Hence $\mathcal{S}_{t+1}$ is a multiset that allows an element to occur more than once. Then the server averages the parameters by $\boldsymbol{\theta}_i^{t+1}=\frac{1}{K} \sum_{k \in \mathcal{S}_{t+1}} \boldsymbol{w}^{t+1}_k$. This sampling scheme is first proposed in \cite{ArXiv_2018_Sahu} but the theoretical analysis was first done in \cite{ICLR_2020_Li_Convergence}.
    \item (\textbf{Scheme II}) The server samples $\mathcal{S}_{t+1}$ uniformly \textbf{\textit{without replacement}}. Hence each element in $\mathcal{S}_{t+1}$ only occurs once. Then the server averages the parameters by $\boldsymbol{\theta}_i^{t+1}=\sum_{k \in \mathcal{S}_{t+1}} p_k \frac{N}{K} \boldsymbol{w}^{t+1}_k$. Note that when the probabilities $\{p_k\}$ are not the same, one cannot ensure $\sum_{k \in \mathcal{S}_{t+1}} p_k \frac{N}{K}=1$ \cite{ICLR_2020_Li_Convergence}.
\end{enumerate}
Pseudo-codes of \texttt{P-FedAvg} are in Appendix \ref{appensec:pseudo_code}.
% \kj{We can add pseudo-code if we have space later.}

\textbf{Communication cost.} The \texttt{P-FedAvg} requires two rounds of communications, aggregation, and broadcast for every $E$ iterations. So at time step $T$, the system completes $2 \lfloor T/E \rfloor$ communications. We follow the setting in \cite{ICLR_2020_Li_Convergence} where the server aggregates based on the chosen scheme and broadcasts the aggregated parameters to all clients. 

Next, we will prove that \texttt{P-FedAvg} has $\mathcal{O}(1/T)$ convergence rate under the above assumption. As a supplement, we prove in Appendix \ref{appensec:alternative} that \texttt{P-FedAvg} also has $\mathcal{O}(1/T)$ convergence rate if we replace Assumption \ref{asm:a5_bound_var_local_grad} with \eqref{asm:uniform_gradnorm_bound}. 


==> Arxiv_ Performative FL (1)/intro.tex <==
\section{Introduction} \label{sec:intro}

Traditional learning problems typically assume data distributions to be static. For applications such as face recognition, this is largely true and designing algorithms under such an assumption in general does not impact learning efficacy.  This,  however, is not true in many other application domains.  In some cases, there may be a natural evolution and shift in the distribution, e.g., in weather and climate data, in which case new data need to be acquired periodically and the algorithm re-trained to remain up to date.  In other cases, the distribution shift is the result of the very learning outcome, when individuals respond to the algorithmic decisions they are subjected to.  For instance, when users with certain accent perceive larger than acceptable error from a speech recognition software and therefore stop using it, this can directly impact the type of speech samples collected by the software used for training the next generation of the product.  Another example is ``gaming the algorithm'', where users through honest or dishonest means attempt to improve critical features so as to obtain a favorable decision by the algorithm (e.g., in loan approval or job application).  This again can directly lead to the distributional change in features and label that the algorithm relies on for decision making. This latter type of distribution shift, one that is a function of the learning model itself, is of particular interest because it has direct implications on how the learning model should be designed. 

Compounding the issue of distribution shift is the issue of data heterogeneity in a distributed learning setting, such as in federated learning (FL).  Distributed learning offers greater privacy protection compared to centralized learning, but distributed data sources can be heterogeneous in nature, and their respective distribution shifts can also be different.  This is particularly the case if one group (a client in the FL architecture) reacts very differently to the learning model, e.g., because it is perceived to be biased against that group.  

In this paper we seek to understand and mitigate the issue of distribution shift in a distributed learning setting, and in particular, the type of shift induced by reactions to the learning model as outlined above.  We will limit our attention to the federated learning architecture. 

There have been a number of approaches studied in the literature to address distribution shift in an FL setting, see e.g., in the contexts of domain adaptation \cite{}, transfer learning \cite{}, and so on. However, the types of distribution shifts considered in these studies typically occur independently of the learning process, whereas we are interested in distribution shifts that are functions of the learning model itself. 

%Traditional learning/prediction problems always treats data distribution as static. While excels in some scenarios such as pattern recognition, when it comes to real world sequential decisions, such prediction models can trigger actions that change the data distribution and influence the prediction objective. This type of predictions are said to be \emph{performative}. Typical examples of performative prediction include \emph{strategic learning} \cite{NEURIPS_2021_Zrnic}, where the decision maker publishes the model first, and the agents move next to strategically manipulate their features and get better decision outcomes, e.g., in credit default risk predictions, applicants will try to manipulate their features to get lower prediction rates and thus lower loan interest rates.

{\em Performative prediction}, first proposed in \cite{ICML_2020_Perdomo_PP} and further developed in a growing literature, see e.g., \cite{NIPS_2020_Mendler, ArXiv_2020_Drusvyatskiy, ArXiv_2020_Brown, AISTATS_2022_Li,IEEE_CSL_2021_Wood,ICML_2021_Zachary,AISTATS_2022_Zachary,ICML_2021_Miller,AAAI_2022_Ray} 
stands out as the appropriate solution concept in this context, whereby the distribution shift is formally captured via a mapping function from the set of model parameters to the space of distributions. However, this  body of literature almost exclusively focuses on a centralized learning setting, with the possible exception of \cite{}. 

%has widely been studied in centralized machine learning. The pioneering work  first formalizes the distribution shift in performative predictions by introducing a distribution mapping function from the set of model parameters to the space of distributions. Later on, a growing literature study the convergence of various algorithms to the stable solution \cite{NIPS_2020_Mendler, ArXiv_2020_Drusvyatskiy, ArXiv_2020_Brown, AISTATS_2022_Li,IEEE_CSL_2021_Wood}, algorithms to find stationary solutions of performative risk \cite{ICML_2021_Zachary,AISTATS_2022_Zachary,ICML_2021_Miller,AAAI_2022_Ray} in centralized performative predictions. 

%However, when it comes to modern large-scale machine learning, centralized model fails due to resource limitation and lack of privacy protection. Thanks to its decentralized schema, federated learning has emerged as an important paradigm. Federated learning allows a large number of clients to collaboratively train a model without data sharing. Many federated learning frameworks are proposed to achieve higher efficiency and better tackling heterogeneity issue\ty{explain.}\cite{mcmahan2017communication, li2020federated, wang2020tackling, karimireddy2020scaffold}. However, none of them address performative\ty{or distribution shift} issue. \xr{i believe there are many FL works addressing distribution shifts (e.g., in contexts of domain adaptation, transfer learning, etc.); to avoid confusion, we should highlight how distribution shifts considered in performative prediction differ from other distribution shifts, i.e., its distribution shifts are functions of model itself}

%Distribution shift can be even more worthy of attention in federated setting. 1) As already being a major difficulty in federated learning, tackling data heterogeneity faces additional challenges when taking disparity of client distribution shift into consideration. 2) During training, clients receive aggregated model at certain steps and train from it. While fitting better as an entity, such aggregation may fail to fit well on each client, which may leads more severe shifting issue. 3) As involving multi parties, clients may be more sensitive about potential shift of other clients and therefore an impact of aggregation model. \ty{more reason? examples like banks loan problem? elaborate?}

%A typical example where we can apply the performative federated learning framework is a bank predicting whether loan applicants are creditworthy. One one hand, the loan applicants have incentives to manipulate their features like the number of credit cards they have, the number of vehicles they own to get a better credit score and thus get the loan. So this becomes a strategic classification problem and can be modeled by performative predictions. On the other hand, these credit related features may involve sensitive information and thus should not be collected by the central server for model training. In this case, we need to apply federated learning algorithms to train the prediction model.

This motivates us to investigate how the performative prediction concept may be used in the FL framework. Specifically, we are interested in whether {\em existing} FL algorithms such as FedAvg \cite{} would converge under distribution shifts modeled in the preformative prediction fashion, and if so, under what conditions. \zc{contradict to the following sentence}

Toward this end, we formally introduce the {\em performative FedAvg} algorithm, or P-FedAvg, and establish its convergence.  Our main findings are as follows. 
\begin{itemize}
    \setlength\itemsep{0.1em}

    \item We are the first work to use the idea of performative predictions to address the distribution shift caused by model decisions in federated learning,  and formalized the performative \texttt{FedAvg} algorithm.
    \item We show that the  \texttt{P-FedAvg} algorithm converges and has a $\mathcal{O}(1/T)$ convergence rate with both the full and partial participation schemes under mild assumptions similar to those in prior works. 
    \item In doing so we also  introduce some novel proof techniques: we prove  convergence without a bounded gradient assumption. This technique can be directly applied to conventional FL, which is a special case of the performative setting.
    \item We prove the uniqueness of the performative stable solution reached by the algorithm, and show that it is a provable approximation to the performative optimal solution under mild conditions. Both solutions will be formally defined in the next section. 
   % \item We prove the uniqueness of the PS solution and show it's close to the PO solution under mild conditions. 
   More interestingly, we show that the stable solution %is not only an approximation to the PO solution, but also 
   has its own game-theoretic interpretation as the fixed point of the best response dynamics. %\xr{we have not introduced the definition of PS \& PO yet; one suggestion is to present part of section 2 in  introduction, e.g., equation (1) and (2); because the reviewers might not have any background in performative prediction, giving formulation earlier can be very helpful.}%\zc{what interpretation}
\zc{experimental results}
%    \item We present novel proof techniques in this paper. In particular, we prove the convergence of performative federated learning algorithms without assuming that the gradient of the loss function is always bounded. This technique can be directly applied to conventional federated learning because conventional setting is just a special case of performative setting.
   % \item Our work can also be regarded as a substantial algorithmic extension to the multi-agent performative prediction \cite{ArXiv_2022_Li_MPP}, since the performative \texttt{FedAvg} supports less frequent communication, partial device participation, and unbalanced clients while achieving the same convergence rate. 
   % \item Our numerical experiments not only validate our theory, showing convergence, reductions in communication time and stragglers' effect, but also show that other federated learning algorithms also empirically converge to the stable solution. \ty{need verify with data heterogeneity.}
\end{itemize}

%To the best of our knowledge, our work is the first to address performative issue in federated learning. We first show that the PS solution is unique and its distance to the performative optimal (PO) solution is bounded. Then we show that FedAvg can guarantee $\mathcal{O}(1/T)$ convergence rate 
% \zc{please note that $\mathcal{O}(1/T)$ is asublinear convergence rate} 
%to the PS solution.
%while significantly reduce communication time and stragglers' effect compared to previous decentralized algorithms. 
%The federated learning algorithm has the following advantages compared to the decentralized algorithm in \cite{ArXiv_2022_Li_MPP}: (1). less frequent communications and aggregations, (2). reducing waiting time in aggregations through random client sampling to improve the computational efficiency, (3). support unbalanced clients.

% Our theoretical analyses center around the \texttt{FedAvg} \cite{} algorithm, where we show linear convergence rate of both the full and partial participation schemes introduced in \cite{} under mild assumptions used in previous works. 
\com{ML: edited through here.  Suggest we cite all key references in the intro but move the related work part to appendix.} 


\ty{HERE.}







\textbf{Related works.} 
\ty{TODO: related work - preformative prediction.}

\textbf{Performative Prediction.}
More recently, \cite{ArXiv_2022_Li_MPP} formalize the multi-agent/player performative predictions where agents try to learn a common decision rule but have heterogeneous distribution shifts (responses) to the model, and study the convergence of decentralized algorithms to the performative stable (PS) solution. The decentralized performative predictions capture the heterogeneity in agents/clients responses to the decision model and avoids centralized data collection for training. However, this work focuses on decentralized setting. 
As discussed above, besides previous works in performative predictions, our work is strongly related to federated learning, especially the convergence study on non-IID clients \cite{ICLR_2020_Li_Convergence}. \kj{todo: expand the discussion to include more works}

\textbf{Strategic Classification and Regression.}
As discussed in \cite{ICML_2020_Perdomo_PP}, performative prediction can be used to solve the repeated strategic classification and regression problems. We can use Stackelberg games to model the strategic classification and regression problems, where the decision maker moves in the first stage by designing, publishing and committing to a decision rule, then the agents move in the second stage, best responding to the decision rule by manipulating their features to get more desirable decision outcomes, and such manipulation can be modeled by the distribution shift mappings in performative predictions. Conventional strategic learning literature focus on finding the Stackelberg equilibrium \cite{}, i.e., the PO solution where the decision maker and the agents know each others' utilities, whereas performative prediction can find the PS solution in repeated strategic learning problems regardless of the knowledge on the utilities.

\textbf{Federated Learning.}
\ty{TODO: related work - fl.}
\begin{itemize}
    \item FedAvg\cite{mcmahan2017communication}. FedProx\cite{li2020federated}, FedNova\cite{wang2020tackling}, Scarffold\cite{karimireddy2020scaffold}, FedGate\cite{haddadpour2021federated}\ty{and personalized fl.}
\end{itemize}

==> Arxiv_ Performative FL (1)/intro_old.tex <==
\section{Introduction(old)} %\label{sec:intro}

Supervised learning excels at pattern recognition when the data distribution is treated as static. However, when it comes to real world sequential decisions, prediction models can trigger actions that change the data distribution and influence the prediction objective. Such predictions are said to be \emph{performative}. Typical examples of performative prediction include \emph{strategic learning} \cite{NEURIPS_2021_Zrnic}, where the decision maker publishes the model first, and the agents move next to strategically manipulate their features and get better decision outcomes, e.g., in credit default risk predictions, applicants will try to manipulate their features to get lower prediction rates and thus lower loan interest rates.

The pioneering work \cite{ICML_2020_Perdomo_PP} first formalizes the distribution shift in performative predictions by introducing a distribution mapping function from the set of model parameters to the space of distributions. Later on, a growing literature study the convergence of various algorithms to the stable solution \cite{NIPS_2020_Mendler, ArXiv_2020_Drusvyatskiy, ArXiv_2020_Brown, AISTATS_2022_Li,IEEE_CSL_2021_Wood}, algorithms to find stationary solutions of performative risk \cite{ICML_2021_Zachary,AISTATS_2022_Zachary,ICML_2021_Miller,AAAI_2022_Ray} in centralized performative predictions. More recently, \cite{ArXiv_2022_Li_MPP} formalize the multi-agent/player performative predictions where agents try to learn a common decision rule but have heterogeneous distribution shifts (responses) to the model, and study the convergence of decentralized algorithms to the performative stable (PS) solution. The decentralized performative predictions capture the heterogeneity in agents/clients responses to the decision model and avoids centralized data collection for training.

In this paper, we introduce federated learning algorithms to solve the decentralized performative prediction problems. To the best of our knowledge, our work is the first to introduce federated learning in performative predictions. We first show that the PS solution is unique and its distance to the performative optimal (PO) solution is bounded. Then we show that federated learning algorithms can guarantee $\mathcal{O}(1/T)$ convergence rate 
% \zc{please note that $\mathcal{O}(1/T)$ is asublinear convergence rate} 
to the PS solution while significantly reduce communication time and stragglers' effect compared to previous decentralized algorithms. The federated learning algorithm has the following advantages compared to the decentralized algorithm in \cite{ArXiv_2022_Li_MPP}: (1). less frequent communications and aggregations, (2). reducing waiting time in aggregations through random client sampling to improve the computational efficiency, (3). support unbalanced clients.

% Our theoretical analyses center around the \texttt{FedAvg} \cite{} algorithm, where we show linear convergence rate of both the full and partial participation schemes introduced in \cite{} under mild assumptions used in previous works. 

We highlight our contributions as follows:
\begin{itemize}
    \setlength\itemsep{0.1em}
    \item We are the first work to address the distribution shift caused by model decisions in federated learning, where we borrow the idea of distribution shift mappings from the performative prediction literature and formalized the performative \texttt{FedAvg} algorithm.
    % \ty{Or, we are the first work to address natural distribution shift in federated learning. From which perspective.}
    \item We prove the uniqueness of the PS solution and show it's close to the PO solution. More importantly, we show that the PS solution is not only an approximation to the PO solution, but also has its own game-theoretic interpretation.
    \item We show that the performative \texttt{FedAvg} algorithm has $\mathcal{O}(1/T)$ convergence rate under both the full and partial participation schemes under mild assumptions used in previous works. 
    \item We provide novel proof techniques in this work. In particular, we prove the convergence of both performative and conventional federated learning algorithms without assuming that the gradient of the loss function is always bounded. 
    \item Our work can also be regarded as a substantial algorithmic extension to the multi-agent performative prediction \cite{ArXiv_2022_Li_MPP}, since the performative \texttt{FedAvg} supports less frequent communication, partial device participation, and unbalanced clients while achieving the same convergence rate. 
    \item Our numerical experiments not only validate our theory, showing convergence, reductions in communication time and stragglers' effect, but also show that other federated learning algorithms also empirically converge to the stable solution. \ty{need verify with data heterogeneity.}
\end{itemize}

\textbf{Related works.} As discussed above, besides previous works in performative predictions, our work is strongly related to federated learning, especially the convergence study on non-IID clients \cite{ICLR_2020_Li_Convergence}. \kj{todo}
\begin{itemize}
    \item FedAvg\cite{mcmahan2017communication}. FedProx\cite{li2020federated}, FedNova\cite{wang2020tackling}, Scarffold\cite{karimireddy2020scaffold}, FedGate\cite{haddadpour2021federated}\ty{and personalized fl.}
\end{itemize}

As discussed in \cite{ICML_2020_Perdomo_PP}, performative prediction can be used to solve the repeated strategic classification and regression problems. Conventional strategic learning literature focus on finding the Stackelberg equilibrium \cite{}, i.e., the PO solution where the decision maker and the agents know each others' utilities, whereas performative prediction can find the PS solution in repeated strategic learning problems regardless of the knowledge on the utilities.

==> Arxiv_ Performative FL (1)/intro_yang.tex <==
\section{Introduction} \label{sec:intro}

Traditional learning problems typically assume data distributions to be static. For applications such as face recognition, this is largely true and designing algorithms under such an assumption in general does not impact learning efficacy.  This,  however, is not true in many other domains.  In some cases, there may be a natural evolution and shift in the distribution, e.g., in weather and climate data, in which case new data need to be acquired periodically and the algorithm re-trained to remain up to date.  In other cases, the distribution shift is the result of the very learning outcome, when individuals respond to the algorithmic decisions they are subjected to.  For instance, when users with certain accents perceive larger-than-acceptable errors from a speech recognition software and therefore stop using it, this can directly impact the type of speech samples collected by the software used for training the next generation of the product.  Another example is ``gaming the algorithm'', where users through honest or dishonest means attempt to improve critical features so as to obtain a favorable decision by the algorithm (e.g., in loan approvals or job applications).  This again can directly lead to the distributional change in features and label that the algorithm relies on for decision making. 

This latter type of distribution shifts, one of particular interest, where
the deployed model itself can trigger changes in the data distribution and influence the objective, said to be \emph{performative}. Performing prediction in the presence of such distribution shift is called \emph{performative prediction} \cite{ICML_2020_Perdomo_PP}. Typical scenarios of performative prediction include \emph{strategic learning} \cite{Hardt2016, dong2018strategic, Milli2019, Hu2019,  braverman2020role, chen2020strategic, pmlr-v119-miller20b, shavit2020causal,Haghtalab2020, Kleinberg2020,NEURIPS_2021_Zrnic}.
% , where agents subjected to model-generated decisions  strategically manipulate their features based on what they know of the  model, in order to obtain better decision outcomes. 
% \com{This feels a bit redundant given strategic manipulation was already explained in the first paragraph, but I suppose this is okay.} 

Performative prediction has been primarily studied in a centralized setting, with fruitful literature including the convergence analysis \cite{NIPS_2020_Mendler, ArXiv_2020_Drusvyatskiy, ArXiv_2020_Brown, AISTATS_2022_Li,IEEE_CSL_2021_Wood} and algorithm development \cite{ICML_2021_Zachary,AISTATS_2022_Zachary,ICML_2021_Miller,AAAI_2022_Ray}.

In modern large-scale machine learning, distributed learning offers greater privacy protection and better avoids the computational resource bottlenecks compared to centralized learning, and federated learning (FL) is one of the most popular examples.
Here the issue of distribution shift is further compounded due to data heterogeneity in a distributed setting. Specifically, the distributed data sources can be heterogeneous in nature, and their respective distribution shifts can also be different.  
Prior works in FL systems that address data distribution shifts, such as \cite{guo2021towards,casado2022concept,DBLP:journals/corr/abs-2002-08782,hosseinalipour2022parallel,zhu2021diurnal,eichner2019semi,ding2020distributed}, typically do not consider shifts in local distributions 
at the client end induced by the model. In this work, we propose the \emph{performative federated learning} framework to study and handle such data shifts in FL. 


Extending the current results in performative prediction to the decentralized FL has a number of challenges. To highlight a few: 1) \emph{Data heterogeneity:} As already one of the major difficulties in FL, tackling data heterogeneity faces additional challenges when taking the disparity of client distribution shift into consideration. 2) \emph{Central $\rightleftarrows$ Local:} During training, clients receive the aggregated model at certain steps and train from it. While fitting better as an entity, such aggregation may fail to fit well on each client, which may lead to more severe shifting issues. 3) \emph{heterogeneity in shift:} some clients may be more sensitive to the deployed decisions and have more drastic data shifts than other clients, e.g., due to different manipulation costs in strategic learning.

Toward this end, we formally introduce the {\em performative FedAvg} algorithm, or \texttt{P-FedAvg}, and establish its convergence.  Our main findings are as follows. 
\begin{itemize}
    \setlength\itemsep{0.1em}

    \item We prove the uniqueness of the performative stable (PS) solution reached by the algorithm, and show that it is a provable approximation to the performative optimal (PO) solution under mild conditions. Both solutions will be formally defined in Section \ref{subsec:system_settings_objectives}. More interestingly, we show that the stable solution has its own game-theoretic interpretation as the fixed point of the best response dynamics. 
    \item We show in Section \ref{subsec:discussion_alg_sol} that the \texttt{P-FedAvg} algorithm converges to the performative stable solution and has a $\mathcal{O}(1/T)$ convergence rate with both the full and partial participation schemes under mild assumptions similar to those in prior works. 
    \item In doing so we also  introduce some novel proof techniques: we prove  convergence without a bounded gradient assumption. This technique can be directly applied to conventional FL, which is a special case of the performative setting.
\end{itemize}

\subsection{Related Works} 

\textbf{Federated Learning.}
Our work is strongly related to the literature on federated learning (FL). Although many studies have tried
to address client heterogeneity in FL through constrained gradient optimization and knowledge
distillation \cite{li2020federated,karimireddy2020scaffold,wang2020tackling,haddadpour2021federated,zhu2021data,li2019fedmd,lin2020ensemble}, most of them still assume the data is static without considering the distribution shifts. To the best of our knowledge, only a few recent works consider distribution shifts in FL \cite{guo2021towards,casado2022concept,DBLP:journals/corr/abs-2002-08782,hosseinalipour2022parallel,zhu2021diurnal,eichner2019semi,ding2020distributed}. For example, \cite{guo2021towards} considered FL with time-evolving clients where the  time-drift of each client is modeled as a \textit{time-independent} additive noise with \textit{zero-mean} and \textit{bounded variance}. \cite{casado2022concept} proposed an FL algorithm adaptable to distribution drifts; it monitors the confidence scores of the model prediction throughout the learning process and assumes the drift happens whenever there is a  substantial drop in confidence scores. \cite{DBLP:journals/corr/abs-2002-08782} also studied dynamic FL and assumed the true model under time-evolving data follows a \textit{random walk}. \cite{hosseinalipour2022parallel} considered FL with dynamic clients and modeled the drift using the variation in \textit{local loss} over two consecutive time steps. \cite{zhu2021diurnal,eichner2019semi,ding2020distributed} considered the \textit{periodical} distribution shift of client population in FL; they assume the
\textit{block-cyclic} structure where the clients from two different time zones alternately participate in training.  

\textbf{Performative Prediction.} In addition to the one we discussed in the introduction that focuses on the centralized setting for performative prediction, more recently, \cite{ArXiv_2022_Li_MPP} formalize the multi-agent/player performative predictions where agents try to learn a common decision rule but have heterogeneous distribution shifts (responses) to the model, and study the convergence of decentralized algorithms to the PS solution. The decentralized performative predictions capture the heterogeneity in agents'/clients' responses to the decision model and avoid centralized data collection for training. This work provides inspiration for our formulation of the performative federated learning framework, and our proposed \texttt{P-FedAvg} can be viewed as a substantial algorithmic extension that supports unbalanced data, much less frequent synchronizations, and partial device participation.
\cite{Narang_2022_ArXiv} propose a decentralized multi-player performative prediction framework where the players react to competing institutions’ actions. \cite{raab2021unintended} proposes a replicator dynamics model with label shift.

\textbf{Strategic Classification and Regression.}
As discussed in \cite{ICML_2020_Perdomo_PP}, performative prediction can be used to solve repeated strategic classification and regression problems. We can use Stackelberg games to model these problems, where the decision maker moves in the first stage by designing, publishing, and committing to a decision rule, then the agents move in the second stage, best responding to the decision rule by manipulating their features to get more desirable decision outcomes, and such manipulation can be modeled by the distribution shift mappings. Conventional strategic learning literature focus on finding the Stackelberg equilibrium \cite{Hardt2016,Kleinberg2020,shavit2020causal,Haghtalab2020}, i.e., the PO solution where the decision maker and the agents know each others' utilities, whereas performative prediction can find the PS solution in repeated strategic learning problems regardless of the knowledge on the utilities.


==> Arxiv_ Performative FL (1)/numerical.tex <==
\section{Numerical Experiments} \label{sec:numerical}

\subsection{Weighted Gaussian mean performative prediction}

As a numerical simulation, we perform \texttt{P-FedAvg} to estimate the mean of heterogeneous Gaussian data under performative effects and examine the impact of the hyperparameters, the sampling schemes, and client heterogeneity. We consider $N = 25$ clients, with the $i$-th client minimizing the loss function $\ell(\theta; Z_i) := (\theta - Z)^2 / 2$, $\theta, Z \in \mathbb{R}$ on data $Z_i\sim \mathcal{D}_i(\theta) := \mathcal{N}(m_i + \epsilon_i \theta, \sigma^2)$. For this loss function, we have $\mu = 1$, $L=1$. For $\overline{\epsilon} \in [0,1)$, the PS solution is $\theta^{PS} = \frac{\sum_{i=1}^N p_i m_i}{1 - \overline{\epsilon}}$; while $\theta^{PS}$ does not exist when $\overline{\epsilon} \geq 1$.  Denote the weighted average of $m_i$ as $\overline{m} = \sum_{i=1}^N p_i m_i$ and the variance as $\text{Var}(m) = \sum_{i=1}^N p_i (m_i - \overline{m})^2$. In experiment, we set $\overline{\epsilon} = 0.9$, $\overline{m} = 10$.


\begingroup

 \begin{figure}
     \centering
     \includegraphics[width=0.45\textwidth]{figures/convergence_g.pdf}
     \caption{Distance to the performative stable solution vs. the number of iterations for full participation, Scheme I, and Scheme II.}
     \label{fig:convergence}
 \end{figure}
 
Figure \ref{fig:convergence} shows \texttt{P-FedAvg} converges to the performative stable solution in all three communication settings: full participation and the two schemes for the partial participation. Interestingly, partial participation with scheme II converges the fastest in this experiment. Despite the full participation scheme having the lowest upper bound on the number of iterations sufficient to convergence, our experimental results show that the actual convergence behaviors of all three schemes are very similar and weakly depend on $K$, especially when $p_i = \frac{1}{N}$.





{\bf Impact of $E$.} We conduct an experiment to compare the performance of our algorithm with a variety of $E$ values, under a homogeneous system. Figure \ref{fig:impactofe} shows the result on both sampling schemes, with $K=20$. A slightly larger $E$ leads to faster convergence. However, an extremely large $E$($E=50$ in the experiment) can also cause slower convergence. Since at this case, the clients deviate too much at each aggregation, which causes low efficiency issues. In real world scenarios, as the communication cost changes, $E$ should be carefully chosen.
 \endgroup
 
\begin{figure}[htbp]
    \centering
    \subfigure[Scheme I]{\label{fig:impactofe:a}\includegraphics[width=0.45\textwidth]{figures/ImpactofE_with.pdf}}
    \subfigure[Scheme II]{\label{fig:impactofe:b}\includegraphics[width=0.45\textwidth]{figures/ImpactofE_without.pdf}}
    \caption{Impact of E on Scheme I and Scheme II. 
    $K=20$, $\text{Var}(m) = 0.6$, $\text{Var}(\epsilon) = 0.1$ for both (a) and (b). For (b), $p_i = \frac{1}{25}$.}
    \label{fig:impactofe}
\end{figure}

{\bf Impact of $K$.} Figure \ref{fig:impactofk} shows the convergence of FedAvg under different k values, For scheme I, larger k leads to faster convergence. While for scheme II, as $k$ increasing, the convergence rate will first increase and then decrease. %Increasing K reduces the value of $B_1, B_2$. 
\begin{figure}[htbp]
    \centering
    \subfigure[Scheme I]{\label{fig:impactofk:a}\includegraphics[width=0.45\textwidth]{figures/ImpactofK_with.pdf}}
    % \hfill
    \subfigure[Scheme II]{\label{fig:impactofk:b}\includegraphics[width=0.45\textwidth]{figures/ImpactofK_without.pdf}}
    \caption{Impact of K on Scheme I and Scheme II . 
    $E=5$, $\text{Var}(m) = 0.6$, $\text{Var}(\epsilon) = 0.1$ for both (a) and (b). For (b), $p_i = \frac{1}{25}$.}
    \label{fig:impactofk}
\end{figure}

{\bf Impact of sampling schemes.} Figure \ref{fig:convergence} also compares different schemes. We can see if the clients' data are uniformly sampled ($p_i = \frac{1}{N}$), then scheme II achieves a better convergence rate, which conforms to our theoretical result because $B_1>B_2$.

{\bf Data heterogeneity and shifting heterogeneity.}
In Figure \ref{fig:impactofh} we test our algorithm under data heterogeneity. Specifically, we set $m$ and $\epsilon$ to have large variances, respectively. In this example, $m$ mainly captures the data heterogeneity and $\epsilon$ capture the shifting heterogeneity. This experiment shows our algorithm still converges under a certain amount of heterogeneity. Comparing the performance of our algorithm on both figures, we can see shifting heterogeneity is the main factor in performative federated learning. 
\begin{figure}[htbp]  
\centering
    \subfigure[Heterogeneity in $m_i$]{\label{fig:impactofh:a}\includegraphics[width=0.45\textwidth]{figures/Impactofmu_h.pdf}}
    % \hfill
    \subfigure[Heterogeneity in $\epsilon_i$]{\label{fig:impactofh:b}\includegraphics[width=0.45\textwidth]{figures/Impactofeps_h.pdf}}
    \caption{Impact of heterogeneity on the two schemes of partial participation. The impact of $m_i$ is shown in (a) and the impact of $\epsilon_i$ is shown in (b). 
    % This experiment is performed on \expg. 
    $K=20, p_i = \frac{1}{25}$ and. In (a), $\text{Var}(m) = 6$ for hetergeneous case and $0$ for homogeneous case, $\text{Var}(\epsilon) = 0.1$. In (b), $\text{Var}(\epsilon) = 0.6$ for hetergeneous case and $0.1$ for homogeneous case, $\text{Var}(m) = 0.6$.}
    \label{fig:impactofh}
\end{figure}

\subsection{Credit Score Strategic Classification}

To show the performance of \texttt{P-FedAvg} on a real world dataset, we follow \cite{ICML_2020_Perdomo_PP} and use the same Kaggle dataset \footnote{www.kaggle.com/competitions/GiveMeSomeCredit/data}, where a bank predicts whether loan applicants are creditworthy. 
The features consist of the information about an individual, and the target is 1 if the individual defaulted on a loan, and 0 otherwise. We use the same strategic setting as in \cite{ICML_2020_Perdomo_PP} where the applicants can manipulate their features in (1) revolving utilization of unsecured lines, (2) number of open credit lines and loans, and (3) number real estate loans or lines. The strength of manipulation for the $i$-th population is controlled by $\epsilon_i$. We equally partition the training set into 10 subsets and distributed it to 10 clients, and thus $p_i = 0.1, \forall i$. The sensitivities $\epsilon_i$ for the 10 clients are independently and uniformly sampled from $[0.9, 1.1]$. We set $K=5$ in partial participation. We train a logistic regression binary classifier. In each round of \texttt{P-FedAvg}, we perform $E=5$ gradient descent steps on a random minibatch of size 4. A discussion on the effect of the batch size can be found in Appendix~\ref{appensec:exp_credit}.

Figure~\ref{fig:credit} shows the loss function and the distance to the PS solution as the number of deployment rounds increases. The mean and 1 standard deviation error bar are generated from 5 experiments with different random seeds. Similar to the numerical simulation, the actual convergence behaviors of all three schemes are very similar.

%% Batch size = 16
\begin{figure} [htbp]
    % \centering
    \subfigure[Training losses]{\label{fig:credit_loss}\includegraphics[width=0.45\textwidth]{figures/credit/b4e5_credit_loss.pdf}}
    % \hfill
    \subfigure[Distances to $\boldsymbol{\theta}^{PS}$]{\label{fig:credit_dtheta}\includegraphics[width=0.45\textwidth]{figures/credit/b4e5_credit_dtheta.pdf}}
    \caption{The losses (a) and the distances to the PS solution (b) for the full participation, Scheme I and Scheme II.}
    \label{fig:credit}
\end{figure}


==> intro.tex <==
\section{Introduction} \label{sec:intro}

Traditional learning problems typically assume data distributions to be static. For applications such as face recognition, this is largely true and designing algorithms under such an assumption in general does not impact learning efficacy.  This,  however, is not true in many other application domains.  In some cases, there may be a natural evolution and shift in the distribution, e.g., in weather and climate data, in which case new data need to be acquired periodically and the algorithm re-trained to remain up to date.  In other cases, the distribution shift is the result of the very learning outcome, when individuals respond to the algorithmic decisions they are subjected to.  For instance, when users with certain accent perceive larger than acceptable error from a speech recognition software and therefore stop using it, this can directly impact the type of speech samples collected by the software used for training the next generation of the product.  Another example is ``gaming the algorithm'', where users through honest or dishonest means attempt to improve critical features so as to obtain a favorable decision by the algorithm (e.g., in loan approval or job application).  This again can directly lead to the distributional change in features and label that the algorithm relies on for decision making. This latter type of distribution shift, one that is a function of the learning model itself, is of particular interest because it has direct implications on how the learning model should be designed. 

Compounding the issue of distribution shift is the issue of data heterogeneity in a distributed learning setting, such as in federated learning (FL).  Distributed learning offers greater privacy protection compared to centralized learning, but distributed data sources can be heterogeneous in nature, and their respective distribution shifts can also be different.  This is particularly the case if one group (a client in the FL architecture) reacts very differently to the learning model, e.g., because it is perceived to be biased against that group.  

In this paper we seek to understand and mitigate the issue of distribution shift in a distributed learning setting, and in particular, the type of shift induced by reactions to the learning model as outlined above.  We will limit our attention to the federated learning architecture. 

There have been a number of approaches studied in the literature to address distribution shift in an FL setting, see e.g., in the contexts of domain adaptation \cite{}, transfer learning \cite{}, and so on. However, the types of distribution shifts considered in these studies typically occur independently of the learning process, whereas we are interested in distribution shifts that are functions of the learning model itself. 

%Traditional learning/prediction problems always treats data distribution as static. While excels in some scenarios such as pattern recognition, when it comes to real world sequential decisions, such prediction models can trigger actions that change the data distribution and influence the prediction objective. This type of predictions are said to be \emph{performative}. Typical examples of performative prediction include \emph{strategic learning} \cite{NEURIPS_2021_Zrnic}, where the decision maker publishes the model first, and the agents move next to strategically manipulate their features and get better decision outcomes, e.g., in credit default risk predictions, applicants will try to manipulate their features to get lower prediction rates and thus lower loan interest rates.

{\em Performative prediction}, first proposed in \cite{ICML_2020_Perdomo_PP} and further developed in a growing literature, see e.g., \cite{NIPS_2020_Mendler, ArXiv_2020_Drusvyatskiy, ArXiv_2020_Brown, AISTATS_2022_Li,IEEE_CSL_2021_Wood,ICML_2021_Zachary,AISTATS_2022_Zachary,ICML_2021_Miller,AAAI_2022_Ray} 
stands out as the appropriate solution concept in this context, whereby the distribution shift is formally captured via a mapping function from the set of model parameters to the space of distributions. However, this  body of literature almost exclusively focuses on a centralized learning setting, with the possible exception of \cite{}. 

%has widely been studied in centralized machine learning. The pioneering work  first formalizes the distribution shift in performative predictions by introducing a distribution mapping function from the set of model parameters to the space of distributions. Later on, a growing literature study the convergence of various algorithms to the stable solution \cite{NIPS_2020_Mendler, ArXiv_2020_Drusvyatskiy, ArXiv_2020_Brown, AISTATS_2022_Li,IEEE_CSL_2021_Wood}, algorithms to find stationary solutions of performative risk \cite{ICML_2021_Zachary,AISTATS_2022_Zachary,ICML_2021_Miller,AAAI_2022_Ray} in centralized performative predictions. 

%However, when it comes to modern large-scale machine learning, centralized model fails due to resource limitation and lack of privacy protection. Thanks to its decentralized schema, federated learning has emerged as an important paradigm. Federated learning allows a large number of clients to collaboratively train a model without data sharing. Many federated learning frameworks are proposed to achieve higher efficiency and better tackling heterogeneity issue\ty{explain.}\cite{mcmahan2017communication, li2020federated, wang2020tackling, karimireddy2020scaffold}. However, none of them address performative\ty{or distribution shift} issue. \xr{i believe there are many FL works addressing distribution shifts (e.g., in contexts of domain adaptation, transfer learning, etc.); to avoid confusion, we should highlight how distribution shifts considered in performative prediction differ from other distribution shifts, i.e., its distribution shifts are functions of model itself}

%Distribution shift can be even more worthy of attention in federated setting. 1) As already being a major difficulty in federated learning, tackling data heterogeneity faces additional challenges when taking disparity of client distribution shift into consideration. 2) During training, clients receive aggregated model at certain steps and train from it. While fitting better as an entity, such aggregation may fail to fit well on each client, which may leads more severe shifting issue. 3) As involving multi parties, clients may be more sensitive about potential shift of other clients and therefore an impact of aggregation model. \ty{more reason? examples like banks loan problem? elaborate?}

%A typical example where we can apply the performative federated learning framework is a bank predicting whether loan applicants are creditworthy. One one hand, the loan applicants have incentives to manipulate their features like the number of credit cards they have, the number of vehicles they own to get a better credit score and thus get the loan. So this becomes a strategic classification problem and can be modeled by performative predictions. On the other hand, these credit related features may involve sensitive information and thus should not be collected by the central server for model training. In this case, we need to apply federated learning algorithms to train the prediction model.

This motivates us to investigate how the performative prediction concept may be used in the FL framework. Specifically, we are interested in whether {\em existing} FL algorithms such as FedAvg \cite{} would converge under distribution shifts modeled in the preformative prediction fashion, and if so, under what conditions. \zc{contradict to the following sentence}

Toward this end, we formally introduce the {\em performative FedAvg} algorithm, or P-FedAvg, and establish its convergence.  Our main findings are as follows. 
\begin{itemize}
    \setlength\itemsep{0.1em}

    \item We are the first work to use the idea of performative predictions to address the distribution shift caused by model decisions in federated learning,  and formalized the performative \texttt{FedAvg} algorithm.
    \item We show that the  \texttt{P-FedAvg} algorithm converges and has a $\mathcal{O}(1/T)$ convergence rate with both the full and partial participation schemes under mild assumptions similar to those in prior works. 
    \item In doing so we also  introduce some novel proof techniques: we prove  convergence without a bounded gradient assumption. This technique can be directly applied to conventional FL, which is a special case of the performative setting.
    \item We prove the uniqueness of the performative stable solution reached by the algorithm, and show that it is a provable approximation to the performative optimal solution under mild conditions. Both solutions will be formally defined in the next section. 
   % \item We prove the uniqueness of the PS solution and show it's close to the PO solution under mild conditions. 
   More interestingly, we show that the stable solution %is not only an approximation to the PO solution, but also 
   has its own game-theoretic interpretation as the fixed point of the best response dynamics. %\xr{we have not introduced the definition of PS \& PO yet; one suggestion is to present part of section 2 in  introduction, e.g., equation (1) and (2); because the reviewers might not have any background in performative prediction, giving formulation earlier can be very helpful.}%\zc{what interpretation}
\zc{experimental results}
%    \item We present novel proof techniques in this paper. In particular, we prove the convergence of performative federated learning algorithms without assuming that the gradient of the loss function is always bounded. This technique can be directly applied to conventional federated learning because conventional setting is just a special case of performative setting.
   % \item Our work can also be regarded as a substantial algorithmic extension to the multi-agent performative prediction \cite{ArXiv_2022_Li_MPP}, since the performative \texttt{FedAvg} supports less frequent communication, partial device participation, and unbalanced clients while achieving the same convergence rate. 
   % \item Our numerical experiments not only validate our theory, showing convergence, reductions in communication time and stragglers' effect, but also show that other federated learning algorithms also empirically converge to the stable solution. \ty{need verify with data heterogeneity.}
\end{itemize}

%To the best of our knowledge, our work is the first to address performative issue in federated learning. We first show that the PS solution is unique and its distance to the performative optimal (PO) solution is bounded. Then we show that FedAvg can guarantee $\mathcal{O}(1/T)$ convergence rate 
% \zc{please note that $\mathcal{O}(1/T)$ is asublinear convergence rate} 
%to the PS solution.
%while significantly reduce communication time and stragglers' effect compared to previous decentralized algorithms. 
%The federated learning algorithm has the following advantages compared to the decentralized algorithm in \cite{ArXiv_2022_Li_MPP}: (1). less frequent communications and aggregations, (2). reducing waiting time in aggregations through random client sampling to improve the computational efficiency, (3). support unbalanced clients.

% Our theoretical analyses center around the \texttt{FedAvg} \cite{} algorithm, where we show linear convergence rate of both the full and partial participation schemes introduced in \cite{} under mild assumptions used in previous works. 
\com{ML: edited through here.  Suggest we cite all key references in the intro but move the related work part to appendix.} 


\ty{HERE.}







\textbf{Related works.} 
\ty{TODO: related work - preformative prediction.}

\textbf{Performative Prediction.}
More recently, \cite{ArXiv_2022_Li_MPP} formalize the multi-agent/player performative predictions where agents try to learn a common decision rule but have heterogeneous distribution shifts (responses) to the model, and study the convergence of decentralized algorithms to the performative stable (PS) solution. The decentralized performative predictions capture the heterogeneity in agents/clients responses to the decision model and avoids centralized data collection for training. However, this work focuses on decentralized setting. 
As discussed above, besides previous works in performative predictions, our work is strongly related to federated learning, especially the convergence study on non-IID clients \cite{ICLR_2020_Li_Convergence}. \kj{todo: expand the discussion to include more works}

\textbf{Strategic Classification and Regression.}
As discussed in \cite{ICML_2020_Perdomo_PP}, performative prediction can be used to solve the repeated strategic classification and regression problems. We can use Stackelberg games to model the strategic classification and regression problems, where the decision maker moves in the first stage by designing, publishing and committing to a decision rule, then the agents move in the second stage, best responding to the decision rule by manipulating their features to get more desirable decision outcomes, and such manipulation can be modeled by the distribution shift mappings in performative predictions. Conventional strategic learning literature focus on finding the Stackelberg equilibrium \cite{}, i.e., the PO solution where the decision maker and the agents know each others' utilities, whereas performative prediction can find the PS solution in repeated strategic learning problems regardless of the knowledge on the utilities.

\textbf{Federated Learning.}
\ty{TODO: related work - fl.}
\begin{itemize}
    \item FedAvg\cite{mcmahan2017communication}. FedProx\cite{li2020federated}, FedNova\cite{wang2020tackling}, Scarffold\cite{karimireddy2020scaffold}, FedGate\cite{haddadpour2021federated}\ty{and personalized fl.}
\end{itemize}

==> intro_old.tex <==
\section{Introduction(old)} %\label{sec:intro}

Supervised learning excels at pattern recognition when the data distribution is treated as static. However, when it comes to real world sequential decisions, prediction models can trigger actions that change the data distribution and influence the prediction objective. Such predictions are said to be \emph{performative}. Typical examples of performative prediction include \emph{strategic learning} \cite{NEURIPS_2021_Zrnic}, where the decision maker publishes the model first, and the agents move next to strategically manipulate their features and get better decision outcomes, e.g., in credit default risk predictions, applicants will try to manipulate their features to get lower prediction rates and thus lower loan interest rates.

The pioneering work \cite{ICML_2020_Perdomo_PP} first formalizes the distribution shift in performative predictions by introducing a distribution mapping function from the set of model parameters to the space of distributions. Later on, a growing literature study the convergence of various algorithms to the stable solution \cite{NIPS_2020_Mendler, ArXiv_2020_Drusvyatskiy, ArXiv_2020_Brown, AISTATS_2022_Li,IEEE_CSL_2021_Wood}, algorithms to find stationary solutions of performative risk \cite{ICML_2021_Zachary,AISTATS_2022_Zachary,ICML_2021_Miller,AAAI_2022_Ray} in centralized performative predictions. More recently, \cite{ArXiv_2022_Li_MPP} formalize the multi-agent/player performative predictions where agents try to learn a common decision rule but have heterogeneous distribution shifts (responses) to the model, and study the convergence of decentralized algorithms to the performative stable (PS) solution. The decentralized performative predictions capture the heterogeneity in agents/clients responses to the decision model and avoids centralized data collection for training.

In this paper, we introduce federated learning algorithms to solve the decentralized performative prediction problems. To the best of our knowledge, our work is the first to introduce federated learning in performative predictions. We first show that the PS solution is unique and its distance to the performative optimal (PO) solution is bounded. Then we show that federated learning algorithms can guarantee $\mathcal{O}(1/T)$ convergence rate 
% \zc{please note that $\mathcal{O}(1/T)$ is asublinear convergence rate} 
to the PS solution while significantly reduce communication time and stragglers' effect compared to previous decentralized algorithms. The federated learning algorithm has the following advantages compared to the decentralized algorithm in \cite{ArXiv_2022_Li_MPP}: (1). less frequent communications and aggregations, (2). reducing waiting time in aggregations through random client sampling to improve the computational efficiency, (3). support unbalanced clients.

% Our theoretical analyses center around the \texttt{FedAvg} \cite{} algorithm, where we show linear convergence rate of both the full and partial participation schemes introduced in \cite{} under mild assumptions used in previous works. 

We highlight our contributions as follows:
\begin{itemize}
    \setlength\itemsep{0.1em}
    \item We are the first work to address the distribution shift caused by model decisions in federated learning, where we borrow the idea of distribution shift mappings from the performative prediction literature and formalized the performative \texttt{FedAvg} algorithm.
    % \ty{Or, we are the first work to address natural distribution shift in federated learning. From which perspective.}
    \item We prove the uniqueness of the PS solution and show it's close to the PO solution. More importantly, we show that the PS solution is not only an approximation to the PO solution, but also has its own game-theoretic interpretation.
    \item We show that the performative \texttt{FedAvg} algorithm has $\mathcal{O}(1/T)$ convergence rate under both the full and partial participation schemes under mild assumptions used in previous works. 
    \item We provide novel proof techniques in this work. In particular, we prove the convergence of both performative and conventional federated learning algorithms without assuming that the gradient of the loss function is always bounded. 
    \item Our work can also be regarded as a substantial algorithmic extension to the multi-agent performative prediction \cite{ArXiv_2022_Li_MPP}, since the performative \texttt{FedAvg} supports less frequent communication, partial device participation, and unbalanced clients while achieving the same convergence rate. 
    \item Our numerical experiments not only validate our theory, showing convergence, reductions in communication time and stragglers' effect, but also show that other federated learning algorithms also empirically converge to the stable solution. \ty{need verify with data heterogeneity.}
\end{itemize}

\textbf{Related works.} As discussed above, besides previous works in performative predictions, our work is strongly related to federated learning, especially the convergence study on non-IID clients \cite{ICLR_2020_Li_Convergence}. \kj{todo}
\begin{itemize}
    \item FedAvg\cite{mcmahan2017communication}. FedProx\cite{li2020federated}, FedNova\cite{wang2020tackling}, Scarffold\cite{karimireddy2020scaffold}, FedGate\cite{haddadpour2021federated}\ty{and personalized fl.}
\end{itemize}

As discussed in \cite{ICML_2020_Perdomo_PP}, performative prediction can be used to solve the repeated strategic classification and regression problems. Conventional strategic learning literature focus on finding the Stackelberg equilibrium \cite{}, i.e., the PO solution where the decision maker and the agents know each others' utilities, whereas performative prediction can find the PS solution in repeated strategic learning problems regardless of the knowledge on the utilities.
